A calibration-free physicality-based model for predicting peak river flows

Many simple hydrologic models are based on parametric statistical relations between the river flow and catchment properties such as its area, precipitation rates, soil properties, etc., fitted to the available data. The main objective of this work is to explain how these statistical relations emerge from the physical laws governing surface and subsurface flow at a catchment scale. The main achievement of this work is the derivation of an analytic formula for predicting peak monthly and annual river flows. It does not require any parameter calibration, but requires a measurement or estimation of the mean flow at the given catchment's outlet. We found that this model 1) has a simple physical interpretation, 2) provides more precise estimates than the median maximum annual flow (QMED) estimation method from the Flood Estimation Handbook (FEH), commonly used to estimate flood risk in the ungauged catchments in the UK, and 3) is highly accurate for all types of catchments, including the small catchments, for which the standard FEH method is the least accurate.

==> TIKZ/seasons_part1.tex <==
\definecolor{fillColor}{RGB}{168,221,181}
\definecolor{lineColor}{RGB}{8,104,172}

\newcommand{\plotgraph}[4] {
   
    
    \begin{axis}[
        mark size=2.9pt,
        width=0.3\linewidth,
        height=0.3\linewidth,
        at={(#3\linewidth, #4\linewidth)},
        xlabel={},
        ylabel={},
        xmin=1e-2,xmax=1e3,
        ymin=1e-2,ymax=1e3,
        xmode = log,
        ymode = log,
        clip marker paths=true,
        axis lines = left,
        axis line style={shorten >=-7pt},
        title={#2},
    ]
    \addplot [color=fillColor, mark=*, only marks, mark size=1pt, opacity=0.4]
    table [x index=0, y index=1, col sep=comma] {DATA/monthly_data/monthly_data_#1.csv};
    \addplot[domain=1e-2:1e3, color=lineColor, line width=1.5pt]{x};
    \end{axis}
}


\begin{tikzpicture}

\plotgraph{1}{January}{0}{0}
\plotgraph{2}{February}{0.3}{0}
\plotgraph{3}{March}{0.6}{0}
\plotgraph{4}{April}{0}{-0.3}
\plotgraph{5}{May}{0.3}{-0.3}
\plotgraph{6}{June}{0.6}{-0.3}
%\plotgraph{7}{July}{0}{0}
%\plotgraph{8}{August}{0.3}{0}
%\plotgraph{9}{September}{0.6}{0}
%\plotgraph{10}{October}{0}{-0.3}
%\plotgraph{11}{November}{0.3}{-0.3}
%\plotgraph{12}{December}{0.6}{-0.3}

\node [anchor=west, scale=0.85, rotate=90] (0) at (-1.2,0) {Measured peak flow};
\node [anchor=west, scale=0.85, rotate=90] (0) at (-1.2,-0.3\linewidth) {Measured peak flow};

\end{tikzpicture}

==> TIKZ/seasons_part2.tex <==
\definecolor{fillColor}{RGB}{168,221,181}
\definecolor{lineColor}{RGB}{8,104,172}

\newcommand{\plotgraph}[4] {
   
    
    \begin{axis}[
        mark size=2.9pt,
        width=0.3\linewidth,
        height=0.3\linewidth,
        at={(#3\linewidth, #4\linewidth)},
        xlabel={},
        ylabel={},
        xmin=1e-2,xmax=1e3,
        ymin=1e-2,ymax=1e3,
        xmode = log,
        ymode = log,
        clip marker paths=true,
        axis lines = left,
        axis line style={shorten >=-7pt},
        title={#2},
    ]
    \addplot [color=fillColor, mark=*, only marks, mark size=1pt, opacity=0.4]
    table [x index=0, y index=1, col sep=comma] {DATA/monthly_data/monthly_data_#1.csv};
    \addplot[domain=1e-2:1e3, color=lineColor, line width=1.5pt]{x};
    \end{axis}
}


\begin{tikzpicture}

\plotgraph{7}{July}{0}{0}
\plotgraph{8}{August}{0.3}{0}
\plotgraph{9}{September}{0.6}{0}
\plotgraph{10}{October}{0}{-0.3}
\plotgraph{11}{November}{0.3}{-0.3}
\plotgraph{12}{December}{0.6}{-0.3}

\node [anchor=west, scale=0.85, rotate=90] (0) at (-1.2,0) {Measured peak flow};
\node [anchor=west, scale=0.85, rotate=90] (0) at (-1.2,-0.3\linewidth) {Measured peak flow};


\node [anchor=west, scale=0.85] (0) at (0,-0.37\linewidth) {Estimated peak flow};
\node [anchor=west, scale=0.85] (0) at (0.3\linewidth,-0.37\linewidth) {Estimated peak flow};
\node [anchor=west, scale=0.85] (0) at (0.6\linewidth,-0.37\linewidth) {Estimated peak flow};

\end{tikzpicture}
